Inclusive Emotion Technologies: Addressing the Needs of d/Deaf and Hard of Hearing Learners in Video-Based Learning

Accessibility efforts for d/Deaf and hard of hearing (DHH) learners in video-based learning have mainly focused on captions and interpreters, with limited attention to learners' emotional awareness--an important yet challenging skill for effective learning. Current emotion technologies are designed to support learners' emotional awareness and social needs; however, little is known about whether and how DHH learners could benefit from these technologies. Our study explores how DHH learners perceive and use emotion data from two collection approaches, self-reported and automatic emotion recognition (AER), in video-based learning. By comparing the use of these technologies between DHH (N=20) and hearing learners (N=20), we identified key differences in their usage and perceptions: 1) DHH learners enhanced their emotional awareness by rewatching the video to self-report their emotions and called for alternative methods for self-reporting emotion, such as using sign language or expressive emoji designs; and 2) while the AER technology could be useful for detecting emotional patterns in learning experiences, DHH learners expressed more concerns about the accuracy and intrusiveness of the AER data. Our findings provide novel design implications for improving the inclusiveness of emotion technologies to support DHH learners, such as leveraging DHH peer learners' emotions to elicit reflections.

==> 6-RQ3.tex <==
% \subsection{RQ3: Factors Impacting Emotional Perception and Experience for DHH}\label{sec:rq3finding} Using interview and self-report(text part). 

% \item \textbf{RQ3}: What are the factors  that contribute to their perceptions and experience?








% Based on interviews provided by the participants, a majority harbored reservations about artificial intelligence, a technology still in its nascent stages of development. Some participants expressed skepticism regarding the AI's accuracy in recognizing facial expressions.










% For example, DPxx said, ``[fill quote here].''
% \haocong{more detailed explanation from DHH vs hearing}







% \subsubsection{Suggestion Towards Better Emotional Experience for DHH}

% We asked participants for further suggestions toward a more inclusive emotional experience in learning. 





% By implementing these strategies, educators can create more inclusive, accessible, and effective learning environments. Such environments enable students to engage more deeply with video-based learning, encourage active participation from all, and facilitate a more comprehensive and nuanced understanding of the subject matter, thereby resonating with the specific needs of each student.




% They suggested including an ASL interpreter to help them better understand the video content than reading captions. In fact, two participants only wrote ``ASL'' as their major concerns and suggestions for the whole learning experience, which they further suggested that they would like to see more ASL included in the video as well as for making self-reports. \haocong{I wonder if there are good quotes that could support this, specifically that they think ASL could help them keep visual attention on video itself and ASL better than captions. If so, this could be a separate paragraph.}

% \jason{Added comparison to hearing, update pid}
% On the other hand, hearing participants have occasionally expressed their concerns about the video presentation with "lack of details and examples" and "lack of consistency" that impacted their experience in learning. % "cohesiveness". % Participants also mentioned that pace of each speaker needs to calibrate in the same level (H7), it distracted the content. % H7: 1:04:30, content can combine, audio,make it feel bored
% In the video, there are multiple speakers who explain different perspectives about AR, each presenting the topic in their own way.
% H11 found that some topics were ``\textit{a bit too high level}'', and ``\textit{would appreciate a bit more in depth.}''
% A new topic was introduced without details, which hindered learners from following the speaker.
% H15 stated that ``\textit{if the example something [is] very relatable that would be really amazing to understand.}``
% H4 realized that visual examples help understanding new concepts and giving more contexts, but ``\textit{the second guy that was talking in the video was not using any visuals.}''



% \haocong{Yes, this is signmaku.}










% \textbf{Summary} %\si{haocong}
% DHH participants expressed lower trust toward AER results, particularly regarding the accuracy of the AI results, the inability to capture internal emotion not expressed on their faces. DHH participants who did not choose emojis in their self-reports found these emojis unable to capture their emotion. Participants also made suggestions toward improving emotional experience, e.g., video presentation styles, peer interactions in often lonely online learning.

==> OLD4-RQ1.tex <==
\section{Findings-RQ1}


\haocong{DHH reported more positive emoji than hearing, and rewatching the video more during self-report, indicating DHH’s learning needs in rewatching for better confidence with multimodal info}

Our analysis on data collected from the in-learning phrase identified challenges in video-based learning for 

%\textit{RQ1:} What are the challenges between DHH students and Hearing College Students for Video-based Learning? (Round 1)
textit{RQ1:} What are the specific challenges that DHH students face with video-based learning in comparison to hearing college students?

\subsection{DHH Expressed More Low Engagement than Hearing Students}\label{sec:rq1finding}

\subsubsection{Self-Report Comparison Quan}
(Self-Report) Feel boring/disengaged ---> lack of engagement

\jason{TODO: A figure to illustrate RQ1 results, such the plot can demonstrate self-report and facial expression data.}
During the in-learning phase, engagement levels were found to be less engaging for DHH participants, which was demonstrated by their increased confusion over facial expression data and use of bored emojis in their self-reports (independent t-test, p<0.05). % need to use of the word significantly
We found that during self-report hearing participants selected emojis in the \textit{+high} quadrant is significantly (t(31)=2.435, p=0.020) more on average compared to the DHH participants, as well as emojis in the \textit{-high} quadrant (t(31)=-2.225, p=0.034).

Result - Hearing participants had more +high and -high reports on average than DHH participants


\subsubsection{Facial Expression Confirms Less Engagement}
(Emotion via Facial Expressions- back up self-reports) DHH students report feeling less engaged and motivated during video-based learning activities compared to hearing college students. 

% did they show a normal distribution
Facial expression data revealed that DHH participant had significantly (t(31)=2.39, p=0.024) more data samples detected as \textit{-high} engagement (e.g. confusion) than the hearing participants.

Result 1 - DHH participants were more in the -high range(e.g. confusion) than hearing participants

44.60730769230769\% of the video,  25.318736842105263\% of the video,

Quad 2 (-High) AI Comparison Between DHH and Hearing: ('Power: 0.78', 'Power: 0.87')

Result 2 - Hearing participants were more in the +low (e.g. relaxed) range than DHH participants

5.244846153846154\% of the video, 19.354684210526315\% of the video,

Quad 4 (+Low) AI Comparison Between DHH and Hearing: ('Power: 0.69', 'Power: 0.80')


\subsubsection{Self-Report Qual- Explaining Factors that negatively/positively impact engagement}

Self-report quotes from DHH reflect/report on perspectives \textbf{NOT} mentioned by hearing: 

\textbf{Instructors' Expression}: P3 self-reported in ASL ``\textit{The woman appears a bit \textbf{stone-faced.} It was boring to watch with such a “bland,” blank face. She didn’t look excited about the AR project. }''

P3 self-reported in ASL ``\textit{It’s interesting to me that this man used his hands more, gesturing, in comparison to the previous woman who had her hands clasped in front of her and was "\textbf{dead-faced.}” The man’s gestures made me feel more connected. I’m more surprised by that.}''

P3 self-reported in ASL ``\textit{I have a similar comment about this part. It was a bit boring.  He doesn't seem very excited about AR like the woman. The previous man seemed excited, but the other two just kinda sit there and talk. Their \textbf{body language} is not engaging. I’m not sure if that has to do with the topic and AR is being transferred into a google headset, and that makes the information more internal and less exciting to them. I don’t know. But he was a \textbf{boring person to watch}.}''


\si{ASL users use facial movements alot --> so they are used to watching ASL users which as lots of facial expressions}

\textbf{Visual Variations}: P8 self-reported in English ``\textit{bright prink shirt, white back ground. Wore my CI, she spoke loudly. Got \textbf{lips} that are readable too.}''

P3 self-reported in ASL ``\textit{It's cool that they showed a \textbf{visualization} of the heavy equipment that got placed on the head. The first computer was heavy and fixed; it was not mobile and could not be brought home. It’s cool to see the technology’s beginning.}''

P6 self-reported in ASL ``\textit{ So, this… really.. Oh, google, I don't use that google phone app, ipixel phone. For me, I wouldn't use it. Cloud phone? Many people may like it, but I would suggest more tech, like more fun, more clear, but the \textbf{animation} is boring to me, it's nothing, I don't feel any interest in this. Maybe they need to \textitbf{add more} something to it? }''

P14 self-reported in English ``\textit{Im curious how it does work on POC people (people of color) because I learned that there is algorithms bias - wonder if \textbf{colors/lights} can regonize POC or different style of room (not simple or blank room)}''   ---- she noticed the colors of environment and people in the video 

P8 self-report in English: ``\textit{I think it's funny how it's ladies first woman, male, male (if that's what they identify by, it's playing by colors too, \textbf{pink, Blue(gray), blue } as in choice of clothing). Video is very old school.}''

P8 self-reported in English ``\textit{AR is supposed to be exciting, \textbf{magical}, not boring. I think I zoned out more than twice.}'' then they reported complaining about the visual information ``\textit{Felt like the video was on a tight budget. Not enough room for creativity.} It doesn't seem visually in English, but her signing shows the visual aspect of it


\textbf{Limited Memory and OverLoad}: P15 self-report in English ``\textit{I'm not a technology person so I'm not very familiar with \textbf{specific names} on the phone, so its really hard for me to be focus or interested in what I'm watching.}''

P15 self-report in English ``\textit{A follow-up to timestamp of 2:29(above), still not understanding what it is that I'm looking at although the video is being displayed showing me what it looks like, its hard for me to process in my head \textbf{which is which}.}'' 

P7 self-report in English: ``\textit{Its actually nice to have a photo to show \textbf{remind you which part} that need to install or repair. we don't have to memory the exactly location.}''

P6 self-reported in ASL ``\textit{So, this AR is like a phone, with a camera, it's good for like to develop designs with technology. Like cartoon TV, not game, its nice to be able to design things for like painting, floor plan, furnitures, its cool to take video of the layout on the floor plan like game, where can move things through technology. Can add animals, through camera, makes it look like real animals, movements. Umm, \textbf{I forgot what else to say}. Umm.. }''

P6 self-reported in ASL ``\textit{ Ok, here. So, this part, what is it? Google.. Umm.. \textbf{forgot name} umm.. (looking at video)...Ok AR for shopping, and for retail. Like back when i was young, it would be good for technology to have to let know to show watches, phone towards to shoes, to help us look at it to see if it looks nice on us, help us know what's our size, and see if clothes and shoes match and fit on us nicely or not match us. }''



\subsubsection{Interview Qual explains the reason for low engagement} Themes below focuses on themes not appeared in the self-report.

\textbf{Lack of Interactivity and Emotion Exchange with Peers and Instructors}

\textit{``The challenge is the lack of interaction and feedback. In traditional classroom-based learning, learners have the opportunity to ask questions, participate in discussions, and receive feedback from their instructors and peers. In video-based learning, there is often little opportunity for interaction, which can make it difficult for learners to stay motivated and engaged.''}

\textit{``For Zoom, I have experienced the challenges such as weak Wifi signal, motivation, and fewer opportunities to interact.''}

P3: ``\textit{Maybe that could be an alternative to the discussion board post where I sign my answer. I could use the tool, provide my emotional responses and sign or type my feedback or both. Something like that would work. But it would need to be in separate from homework and assignments. It would be expressing our emotions, like complaining about our homework after class. I don't know. It might be good for an observation project or something where you watch the teacher’s lecture and then offer your feedback to the teacher. “Oh they were bored, that’s fine. I can change that part of the presentation.” Or maybe it is better between the teachers and less for the students. }''

\textbf{Captions are Boring compared to Visual Variations} P3: ``\textit{...CDIs(Certified Deaf Interpreters)  are skilled at matching facial expressions. For example, that first woman presenter was so bland. The CDI can show that. The CDIcan show that. Hearing people can hear her talk and if she has an accent. I can’t hear that. Maybe she actually sounds excited. I wouldn't know. ... “Does she even like her job? She is \textbf{emotionless}.”..Is that her tone of voice? I don't know. But it’s possible she sound excited in her tone of voice but not physically showing that. That is why ASL is needed. An interpreter or a CDI can provide that information. It would be nice to know what her tone was. Did she have flat affect? Maybe what I saw to be an engaging second presenter in fact sounded flat, and I am mistaken. So, yes I think ASL needs to be included.}''


\subsection{DHH Immediately Rewatched to Increase Confidence, while Hearing Did Not}

\subsubsection{Rewatching Behavior during Self-Report} \si{@Jason}
In comparison to hearing college students, DHH college students exhibit distinct behaviors during the process of providing self-reports.
Specifically, DHH college students showed a combination of video re-watching and self-reporting activities, whereas hearing college students primarily focused on submitting their self-reports.
When it came to video re-watching behaviors, DHH college students devoted considerable time to reviewing specific segments of the video before submitting their self-reports.
In contrast, hearing college students spent less time re-watching the video, mainly using it as a quick verification of the content.
Notably, hearing college students occasionally re-watched brief segments of the video to confirm the correct timestamp, which differed from the re-watching behavior observed among DHH college students.
Following the submission of a self-report, hearing college students frequently skipped to the next timestamp in search of the next self-report, while DHH college students resumed the video without seeking to move backward or forward to the next timestamp.
Additionally, DHH college students often allocated time to reading captions, whereas this step was not undertaken by hearing college students.

\subsubsection{Interview}

\textbf{Improve Confidence} 

Display some quotes: \textit{``It sometimes does not provide a good visual timing for me to look and CC were fast, had to stop few times to just look at graphic image''}

\textit{``The playback and the time speed is a huge help when learning with video-based learning. Gives me time to go back and research a little deeper into what it means and so on and forth.''}

P3: ``\textit{I think it benefits students, not just socially, but personally for self-analysis. It’s a good tool to see patterns in my emotions because if I am constantly negative, that will affect my learning. You know that you’re not in a good mood. It can save all my emotional responses. And I can see that I’m not good, I’m not happy. I can see and visually track that pattern. And it wouldn't be just from boredom, a bad day, or a bad week. I think its a good tool for psychologists. And it’s really nice for my memory. I like the tool for that reason because I struggle with my memory, which makes it hard to remember everything. So this is nice because I can review, look at my emotions, and it helps.}''


==> OLD5-RQ2.tex <==
\section{Findings-RQ2}


\haocong{Overall distribution is the same, but when reviewing temporal, we noticed difference between talking head and non talking head}


T17 \textit{``P17: Yes, thank you. I think COVID really impacted, so taking ZOOM was so hard. This is more of a self-paced system, so I have more control of my learning, my own time. I like the feedback comments, to see who watched it already and help understand the concept of the video. With AI… very interesting. ''}

\textit{RQ2:} What differs between DHH students and Hearing College Students in Reflection for Video-based Learning? (Round 1 + 2 )

\si{have a small paragraph that has the similarity between hearing and DHH, also some briefly summarize from hearing, more balanced study}

Researchers observed a common behavior among both deaf and hearing (DHH) and hearing students, wherein they review their own emotional intensity graph in conjunction with the spots where their peers provide common feedback.
Another shared behavior among both groups of students is expressing boredom on a common peer's comment that indicates a bored state about the video learning content.

\subsection{Less Meta-cognition Expressed and Perceived by the DHH compared to Hearing}\label{sec:rq2finding}

In the context of think-aloud, meta-cognition processes encompass both navigating the learning dashboard (on peers' affects, AI-recognized intensity graph, and self-report ) and verbally articulating sentences to reflect learning experiences in relation to the video content.
\jason{We can't use spoken sentences for DHH, what would be a better word.}
These actions, specifically engaging actively with the learning dashboard and expressing thoughts through spoken sentences, led to the identification of two distinct types of data: behavioral data and perceived data.

To annotate the behavioral data, researcher analyzed the interactions of college students within the learning dashboard, which allowed them to identify four distinct types of interactions that occurred during the meta-cognition processes.


\begin{itemize}
    \item \textit{Rewinding and Fast-Forwarding} - Students utilized the rewind and fast-forward functions within the video player to review through the learning content.
    \item \textit{Checking Own Graph} - Students engaged with their own intensity graph.
    \item \textit{Checking Peers' Affects} - Students reviewed peers' affects.
\end{itemize}

To annotate the perceived data, researchers employed three meta-cognitive processes as identified by X et al.: namely, recalling to articulate personal experiences, expressing agreement or disagreement with peers, and collaboratively constructing shared knowledge.
Each sentence can only be associated with a single behavioral code and a single perceived code.

During the analysis of the think-aloud data, researchers successfully identified and eliminated outliers found in both the behavior data, which encompassed actions like Rewinding and Fast-Forwarding, Checking Own Graph, and Checking Peers' Affects, and the perception data, specifically involving Recalling to Articulate Personal Experiences, as exhibited by the college students. To further explore the differences in meta-cognitive processes between deaf and hard of hearing (DHH) students and their hearing counterparts, two-tailed Mann-Whitney U tests were conducted.
The analyzed results are presented below.



%Same Reflection Processes collect during Think-aloud- A1-B4
% CSCW Explain the codebook


\begin{figure}[h]
\centering
    \begin{minipage}{1\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figure/boxplot_rq2.png}
    \caption{This box plot demonstrates the two statistical significant (p < 0.05) findings via the two-tailed Mann-Whitney U test unveiled in the think-aloud process. Hearing college students present higher mean (M=7.30, SD=6.21) in constructing shared knowledge than DHH individuals (M=0.53, SD=0.74). Additionally, hearing college students present higher mean (M=13.47, SD=10.36) in checking peers' cue than DHH individuals (M=3.0, SD=1.79).}
    \end{minipage}
\end{figure}

\subsubsection{(think-aloud) DHH Reflect Less with Peers' Affects}
\si{@Jason} A4, B4 
We conducted a comparison of the total number of reflexive sentences in the perception data between DHH individuals and college students.
More specifically, we annotated the spoken sentences generated by hearing participants or those translated from ASL, utilizing the three meta-cognitive processes outlined by X et al.
The two-tailed Mann-Whitney U test revealed that hearing college students' perception of collaboratively constructing shared knowledge was statistically significantly higher in mean (M=7.0, SD=6.21) than the DHH college students (M=0.53, SD=0.74) (U = 439.5, p < .001).

In addition to the perception data, we were interested the behavioral interaction occurring during the time when the college students uttered the spoken sentences.
The results of the two-tailed Mann-Whitney U test found that the hearing college students' behavior of checking peers' affects was statistically significantly higher in mean (M=13.47, SD=10.36) than the DHH college students (M=3.0, SD=1.79) (U = 375, p < .001).

These results indicate that DHH college students pay less attention to their peers' affect and engage in less reflection on the ideas of their peers.

\subsubsection{(think-aloud)DHH has fewer Total Sentences and More Distraction}
\si{@ Jason} A5, total

During think-aloud processes, DHH college students (N=13) verbalized on average of 7.61 spoken sentences, while hearing college students (N=38) verbalized on average of 15.84 spoken sentences.
The results of T-test showed there are significant difference (p < .005) between DHH and hearing colleges for the total number of verbalized spoken sentences.
Due to low average spoken sentences among the DHH college students, researchers identified a pattern of distraction where the spoken sentences were found to be unrelated to the learning content.
But this behavior is not observed among hearing college students.

\si{quotes here}
For example, P1 ``Yeah, it’s complex (viewing the peer comment about the system looking complicated). ... \textit{In “8” (8th grade?), I would make an appointment with the teacher to sit and discuss feedback on my work to better understand and I’ve had interpreters through Zoom when the teacher is hearing (non-signer)."}

P3: ``I didn’t think that. Content. ... \textit{Now I’m thinking about my food.} ... I look bored''.%\si{you need the sentence before and after to show they are distracted}

\subsubsection{(Survey) DHH perceived the tool less useful for meta-cognition than hearing} \si{Si}

(Usefulness) DHH found the tool less useful for metacognition than hearing participants in 3 questions

“This tool can help me worry less in order to work well  in video-based learning”

“This tool can help me be constantly aware of my thinking  in video-based learning”

“This tool can help me monitor my thoughts video-based learning.”

\subsection{Reason for Less Reflection and Meta-Cognition} 


\subsubsection{(Survey) (Interview) Limited Exposure to Large Scale Learning Settings}

\textbf{Privacy} DHH disagreed with privacy concerns elicited by navigating peers’ emotions while hearing participants slightly agreed with privacy concerns



Due to their limited access to large-scale learning, and for online learning systems, deaf students do not aware of the scope and potential harm of large-scale AI, and thus do not perceive privacy concerns.

P3``\textit{Yes, a class already knows each other. I don’t think that would be an issue because people are already familiar with each other. They see each other in class. So whether they know each other’s history or not, they’re in the same class. I think its a good idea. }''




\subsubsection{(Interview) Unmet Real-time Social Connectedness Needs} 
DHH believes that post-learning reflections with peers' affects are not genuine interactions and emphasizes the need for real-time engagement with others. They only liked their peers' comments as it seems more real

P3: ``\textit{ I could view my peers’ comments. That gave me a different perspective to consider. I liked seeing those other perspectives. I liked seeing those perspectives from my peers even if they differed from mine because everyone has varying perspectives. That shows their authenticity. I liked that it showed the same video from our differing perspectives. I trust that. Yeah… }''


\subsubsection{(Interview) Lack of AI Literacy and Require Deaf Representation in Explaining AI}

During the interview(after think-aloud and survey), we asked them why they had less think-aloud. Their challenges can be synthesized into several themes


- Don't understand what AI does, it is good, how to use it.  DHH oversimplifies the concept of AI by equating emotion recognition AI with the facial recognition technology used by iPhones for unlocking the phone. They fail to acknowledge the potential inaccuracies of AI and its actual functionalities. 

- Deaf representation. P3 ``\textit{ I think it’d be cool if you used a Deaf person as an example. It would help visualize how to think from a Deaf perspective. To give an example of the emotions, of how to do that method. For example, in class you explain and discuss, but not everyone has access to that kind of conversation, so if you use a Deaf person as an example, the Deaf students can relate. They see how to sign the information, to explain that information. It might require a different process of thinking or… I like your example. I like to see examples. It’s a good example. I want more examples showing Deaf people thinking and expressing themselves in ASL. }''


\subsection{Follow-up Survey and Interview to Understand XAI to Enhance Reflections} \si{Move to discussion}

\href{https://docs.google.com/forms/d/1-d6sZhqLyoQrhRBEzoqSdNBHI5VEEl5Pcog825eCX8Y/edit#responses}{A Google Docs Link}

I answered the frequently asked questions. The question and answer pair they liked the most is "how to use AI for reflections"

5/6 said they feel they learned more about the tool.

3/6 said they found the tool more useful for meta-cognition.

I compared their before-explanation answer and post-explanation answer(within the subject) to the same ethical question. I know that is a small number. 

\textbf{Privacy concerns}: 4/6 changed their perceptions, 2 increased concern, 2 decreased

\textbf{Trust}: 4/6 changed their perceptions, 3 increased, 1 decreased

\textbf{sense of agency}: 4/6 changed their perception, 4 increased, 1 decreased

\textbf{understand limitation of AI}:  3/6 changed their perceptions, 2 increased understandings, 1 decreased understandings

Though I cannot make a conclusion for each dimension, I can probably say, their perceptions changed with different ways. 


\si{to ask Wei about "why" on Friday, can get some really good quotes}

Side Notes, a participant said my explanation does not explain why it is be used by/for deaf: " No, I personally think that AI will never be capable of recognizing deaf expressions"




